Non-invasive multigrid for semi-structured grids

Multigrid solvers for hierarchical hybrid grids (HHG) have been proposed to promote the efficient utilization of high performance computer architectures. These HHG meshes are constructed by uniformly refining a relatively coarse fully unstructured mesh. While HHG meshes provide some flexibility for unstructured applications, most multigrid calculations can be accomplished using efficient structured grid ideas and kernels. This paper focuses on generalizing the HHG idea so that it is applicable to a broader community of computational scientists, and so that it is easier for existing applications to leverage structured multigrid components. Specifically, we adapt the structured multigrid methodology to significantly more complex semi-structured meshes. Further, we illustrate how mature applications might adopt a semi-structured solver in a relatively non-invasive fashion. To do this, we propose a formal mathematical framework for describing the semi-structured solver. This formalism allows us to precisely define the associated multigrid method and to show its relationship to a more traditional multigrid solver. Additionally, the mathematical framework clarifies the associated software design and implementation. Numerical experiments highlight the relationship of the new solver with classical multigrid. We also demonstrate the generality and potential performance gains associated with this type of semi-structured multigrid.

==> fig/hhg_meshes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% author: Matthias Mayr %%
%% date: 03/2018         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tikzpicture}[scale=0.25,node distance=0.2cm]

% some global definitions
\def\hcoarse{9.0} % length of element edge on original coarse grid
\def\hmed{3.0} % length of element edge on medium grid
\def\hfine{1.0} % length of element edge on fine grid
\def\x{0.0} % x-coordinate of bottom left corner
\def\y{0.0} % y-coordinate of bottom left corner

\def\dist{1.5}

% original coarse mesh

% square element
\draw [domainline,fill=blue!20] (\x,\y) -- (\x+\hcoarse,\y) -- (\x+\hcoarse,\y+\hcoarse) -- (\x,\y+\hcoarse) -- cycle;

% triangular element
\draw [domainline,fill=green!20] (\x+\hcoarse,\y) -- (\x+2*\hcoarse,\y+0.5*\hcoarse) -- (\x+\hcoarse,\y+\hcoarse) -- cycle;

% interface
\draw [domainline,color=red] (\x+\hcoarse,\y-\dist) -- (\x+\hcoarse,\y+\hcoarse+\dist);

% notations
\node at (\x+\hcoarse/2,\y+\hcoarse/2) {$\region{\dom}{1}$};
\node at (\x+\hcoarse + \hcoarse/3,\y+\hcoarse/2) {$\region{\dom}{2}$};
\node [right] at (\x+\hcoarse,\y+\hcoarse+\dist) {$\Bound$};

%% domain with mesh
% First refinement
\begin{scope}[shift={(2.5*\hcoarse,0)}]

  % square element
  \draw [domainline,fill=blue!20] (\x,\y) -- (\x+\hcoarse,\y) -- (\x+\hcoarse,\y+\hcoarse) -- (\x,\y+\hcoarse) -- cycle;

  % triangular element
  \draw [domainline,fill=green!20] (\x+\hcoarse,\y) -- (\x+2*\hcoarse,\y+0.5*\hcoarse) -- (\x+\hcoarse,\y+\hcoarse) -- cycle;

  %% square domain
  \foreach \x in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\x,\hcoarse);
  \foreach \y in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\hcoarse,\y);

  %% Triangle
  % outer boundary
	\draw [domainline] (\x+\hcoarse,\y) -- (\x+2*\hcoarse,\y+0.5*\hcoarse) -- (\x+\hcoarse,\y+\hcoarse);
	% vertical lines
	\draw [domainline] (\x+\hcoarse+1*\hmed,\y+1/2*\hmed) -- (\x+\hcoarse+1*\hmed,\y+\hcoarse-1/2*\hmed);
	\draw [domainline] (\x+\hcoarse+2*\hmed,\y+2/2*\hmed) -- (\x+\hcoarse+2*\hmed,\y+\hcoarse-2/2*\hmed);
	% tilted lines
	\draw [domainline] (\x+\hcoarse+2*\hmed,\y+2*\hmed) -- (\x+\hcoarse,\y+\hmed) -- (\x+\hcoarse+\hmed,\y+1/2*\hmed);
	\draw [domainline] (\x+\hcoarse+\hmed,\y+5/2*\hmed) -- (\x+\hcoarse,\y+2*\hmed) -- (\x+\hcoarse+2*\hmed,\y+\hmed);

  % interface
  \draw [domainline,color=red] (\x+\hcoarse,\y-\dist) -- (\x+\hcoarse,\y+\hcoarse+\dist);

\end{scope}

% Second refinement
\begin{scope}[shift={(5*\hcoarse,0)}]

  % square element
  \draw [domainline,fill=blue!20] (\x,\y) -- (\x+\hcoarse,\y) -- (\x+\hcoarse,\y+\hcoarse) -- (\x,\y+\hcoarse) -- cycle;

  % triangular element
  \draw [domainline,fill=green!20] (\x+\hcoarse,\y) -- (\x+2*\hcoarse,\y+0.5*\hcoarse) -- (\x+\hcoarse,\y+\hcoarse) -- cycle;

  %% square domain
  \foreach \x in {0,1.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\x,\hcoarse);
  \foreach \y in {0,1.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\hcoarse,\y);

  %% Triangle
  % outer boundary
	\draw [domainline] (\x+\hcoarse,\y) -- (\x+2*\hcoarse,\y+0.5*\hcoarse) -- (\x+\hcoarse,\y+\hcoarse);
	% vertical lines
  \draw [domainline] (\x+\hcoarse+1*\hfine,\y+1/2*\hfine) -- (\x+\hcoarse+1*\hfine,\y+\hcoarse-1/2*\hfine);
  \draw [domainline] (\x+\hcoarse+2*\hfine,\y+2/2*\hfine) -- (\x+\hcoarse+2*\hfine,\y+\hcoarse-2/2*\hfine);
  \draw [domainline] (\x+\hcoarse+3*\hfine,\y+3/2*\hfine) -- (\x+\hcoarse+3*\hfine,\y+\hcoarse-3/2*\hfine);
  \draw [domainline] (\x+\hcoarse+4*\hfine,\y+4/2*\hfine) -- (\x+\hcoarse+4*\hfine,\y+\hcoarse-4/2*\hfine);
  \draw [domainline] (\x+\hcoarse+5*\hfine,\y+5/2*\hfine) -- (\x+\hcoarse+5*\hfine,\y+\hcoarse-5/2*\hfine);
  \draw [domainline] (\x+\hcoarse+6*\hfine,\y+6/2*\hfine) -- (\x+\hcoarse+6*\hfine,\y+\hcoarse-6/2*\hfine);
  \draw [domainline] (\x+\hcoarse+7*\hfine,\y+7/2*\hfine) -- (\x+\hcoarse+7*\hfine,\y+\hcoarse-7/2*\hfine);
  \draw [domainline] (\x+\hcoarse+8*\hfine,\y+8/2*\hfine) -- (\x+\hcoarse+8*\hfine,\y+\hcoarse-8/2*\hfine);
	% tilted lines
	\draw [domainline] (\x+\hcoarse+1*\hfine,\y+1/2*\hfine) -- (\x+\hcoarse,\y+1*\hfine) -- (\x+\hcoarse+8*\hfine,\y+\hcoarse-8/2*\hfine);
	\draw [domainline] (\x+\hcoarse+2*\hfine,\y+2/2*\hfine) -- (\x+\hcoarse,\y+2*\hfine) -- (\x+\hcoarse+7*\hfine,\y+\hcoarse-7/2*\hfine);
	\draw [domainline] (\x+\hcoarse+3*\hfine,\y+3/2*\hfine) -- (\x+\hcoarse,\y+3*\hfine) -- (\x+\hcoarse+6*\hfine,\y+\hcoarse-6/2*\hfine);
	\draw [domainline] (\x+\hcoarse+4*\hfine,\y+4/2*\hfine) -- (\x+\hcoarse,\y+4*\hfine) -- (\x+\hcoarse+5*\hfine,\y+\hcoarse-5/2*\hfine);
	\draw [domainline] (\x+\hcoarse+5*\hfine,\y+5/2*\hfine) -- (\x+\hcoarse,\y+5*\hfine) -- (\x+\hcoarse+4*\hfine,\y+\hcoarse-4/2*\hfine);
	\draw [domainline] (\x+\hcoarse+6*\hfine,\y+6/2*\hfine) -- (\x+\hcoarse,\y+6*\hfine) -- (\x+\hcoarse+3*\hfine,\y+\hcoarse-3/2*\hfine);
	\draw [domainline] (\x+\hcoarse+7*\hfine,\y+7/2*\hfine) -- (\x+\hcoarse,\y+7*\hfine) -- (\x+\hcoarse+2*\hfine,\y+\hcoarse-2/2*\hfine);
	\draw [domainline] (\x+\hcoarse+8*\hfine,\y+8/2*\hfine) -- (\x+\hcoarse,\y+8*\hfine) -- (\x+\hcoarse+1*\hfine,\y+\hcoarse-1/2*\hfine);
	
  % interface
  \draw [domainline,color=red] (\x+\hcoarse,\y-\dist) -- (\x+\hcoarse,\y+\hcoarse+\dist);

\end{scope}

    
%%% description
%% domain
%\node [above] at (\lf+\gap/2,\h+\myspace) {$\FSII$};
%\node [above] at (\lf/2,\h+\myspace) {$\flu{\dom}$};
%\node [above] at (\lf+\gap+\ls/2,\h+\myspace) {$\str{\dom}$};
%% procs
%\node [below,draw,rounded rectangle,fill=red!20] (2) at (0.65*\lf,-2*\myspace) {proc $1$};
%\node [left=of 2,draw,rounded rectangle,fill=green!20] (1) {proc $0$};
%\node [right=of 2,draw,rounded rectangle,fill=blue!20] (3) {proc $2$};
%\node [right=of 3,draw,rounded rectangle,dashed,very thick] (4) {physical fields};

  
\end{tikzpicture}




==> fig/oneDimProblem.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% author: Matthias Mayr %%
%% date: 03/2018         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tikzpicture}[scale=1.0,node distance=0.2cm]

% some global definitions
\def\r{2pt} % radius of dots in V-cycles

\foreach \x in {0,0.5,...,6}
  \filldraw [black] (\x,0) circle [radius=\r];
  
\draw [domainline] (0,0) -- (6.1,0);
\draw [domainline, dashed] (6.2,0) -- (7.2,0);

\foreach \x in {7.4,7.9,...,9.4}
  \filldraw [black] (\x,0) circle [radius=\r];
  
\draw [domainline] (7.3,0) -- (9.4,0);

% notations
\draw [domainline,decoration={brace,amplitude=4,mirror,raise=5},decorate] (0.0,0) -- node[below=0.3] {$\region{\dom}{1}$} (1.5,0);
\draw [domainline,decoration={brace,amplitude=4,mirror,raise=5},decorate] (1.5,0) -- node[below=0.3] {$\region{\dom}{2}$} (4.5,0);
\draw [domainline,decoration={brace,amplitude=4,mirror,raise=5},decorate] (4.5,0) -- node[below=0.3] {$\region{\dom}{3}$} (6.3,0);
\draw [domainline,decoration={brace,amplitude=4,mirror,raise=5},decorate] (6.3,0) -- node[below=0.3] {$\region{\dom}{\indReg}$} (6.9,0);
\draw [domainline,decoration={brace,amplitude=4,mirror,raise=5},decorate] (6.9,0) -- node[below=0.3] {$\region{\dom}{\numReg}$} (9.4,0);


  
\end{tikzpicture}




==> fig/twoDimProblem.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% author: Matthias Mayr %%
%% date: 03/2018         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tikzpicture}[scale=0.25,node distance=0.2cm]

% some global definitions
\def\hcoarse{9.0} % length of element edge on original coarse grid
\def\hmed{3.0} % length of element edge on medium grid
\def\hfine{1.0} % length of element edge on fine grid
\def\x{0.0} % x-coordinate of bottom left corner
\def\y{0.0} % y-coordinate of bottom left corner

\def\dist{0.25}
\def\myspace{0.5}

% bottom left region
\begin{scope}[shift={(0,0)}]

	\draw [domainline,fill=red!20] (0,0) -- (9,0) -- (9,9) -- (0,9) -- cycle;
	
  \foreach \x in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\x,\hcoarse);
  \foreach \y in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\hcoarse,\y);

\end{scope}

% bottom right region
\begin{scope}[shift={(9,0)}]

	\draw [domainline,fill=blue!20] (0,0) -- (9,0) -- (9,9) -- (0,9) -- cycle;

  \foreach \x in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\x,\hcoarse);
  \foreach \y in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\hcoarse,\y);

\end{scope}

% top left region
\begin{scope}[shift={(0,9)}]

	\draw [domainline,fill=cyan!20] (0,0) -- (9,0) -- (9,9) -- (0,9) -- cycle;

  \foreach \x in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\x,\hcoarse);
  \foreach \y in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\hcoarse,\y);

\end{scope}

% top right region
\begin{scope}[shift={(9,9)}]

	\draw [domainline,fill=green!20] (0,0) -- (9,0) -- (9,9) -- (0,9) -- cycle;

  \foreach \x in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\x,\hcoarse);
  \foreach \y in {0,3.0,...,9.0}
    \draw [domainline] (\x,\y) -- (\hcoarse,\y);

\end{scope}
  
\end{tikzpicture}




==> transferOp.tex <==
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "region_multigrid"
%%% End: 

\textbf{Outline of the transfer operator work needed for the paper}
The work consists of two main algorithmic areas: work on aggregation algorithms, this will be Peter's responsibility, and work on the prolongators, basically there is a need for a prolongator factory that will replace the current TentativePFactory from our XML input deck on purely structured grids, this will be Luc's responsibility.\\
The due date associated with each item is subject to modification depending on implementation difficulties and conferences, but it seems realistic and allows for time before the end of the summer to perform testing on examples of interest as well as to write up things before Peter leaves.
\begin{enumerate}
  \item Aggregation for structured/unstructured meshes
    \begin{enumerate}
    \item \todo{Peter}{Interface aggregation phase, due June 19th}\\
      Adding new phase to uncoupled aggregation that aggregates an interface based on a list of coarse points (specified by GID or LID?). This phase is called first before any other phases and it forms aggregates using the nodes in the coarse points list as roots for aggregates. So far we simply aggregate all the neighbors of a root point in an aggregate with said root point. However it is not impossible to have leftover nodes on the interface with this approach, is it a problem? Also the aggregates on both side of the interface will not match, only the root nodes will, is that also a problem? Finally we are currently assuming that the list of interface root nodes is passed as a map, but we should decide what makes most sense during our next meeting.\\
      \pohm{I have integrated the Interface aggregation phase into \muelu. It currently requires the ``aggregation: use interface aggregation'' parameter list flag as well as an array similar to the dirichletBoundaryMap that flags whether or not a node should be forced to be a root node. What I need now is to know how the list of interface root nodes is going to be passed.}
    \item \todo{Peter}{Hybrid aggregation, due July 3rd, maybe 17th}\\
      Create a new aggregation factory (HybridAggregationFactory?) that is able to decide whether the local mesh is aggregated using structured aggregation or using uncoupled aggregation. The idea here is to have the application add a parameter on the \muelu parameter list that tells us which algorithm to use. Based on that parameter, the factory will choose the proper sub-list of parameters and construct the aggregation algorithm. For this task we will use a simple driver that has two uncoupled regions, one will be treated as structured and the other one will be treated as unstructured. We do not need to use the "Interface" phase of aggregation to finish this task.
      \pohm{HybridAggregationFactory has been added, it needs a parameter that specifies what type of aggregation (uncoupled or structured) to use and call the respective ``buildAggregates'' factories. We need to consider how Dirichlet boundary conditions are handled, as unstructured uncoupled aggregation handles Dirichelt points by not aggregating them and structured aggregation has no special handling for Dirichelt points.}
    \item \todo{Peter}{Region structured/unstructured aggregation, due Aug 14th} Here the idea is to combine the above two tasks and to have a mesh that has an interface replicated on two ranks. One region will be treated as structured and the other will be treated as unstructured. The challenge here will be to have the aggregation on both region match along an interface that will be specified by the driver application.
    \end{enumerate}
  \item Prolongators for structured aggregation
    \begin{enumerate}
    \item \todo{Luc}{update aggregate class for overlapping aggregates, due June 19th}\\
      Currently the aggregates class holds a vector called \texttt{vertex2AggId} of size \texttt{numNodes}, which tells each fine node its assigned aggregate. For piece-wise constant aggregation this makes sense as a fine nodes is associated with a single coarse node. However for piece-wise linear interpolation a fine node is associated to it closest neighboring coarse node. The aggregate class needs to be modified in order to store the ID of more than one coarse node per fine node.
    \item \todo{Luc}{add linear interpolation capability to structures aggregation, due July 3rd}\\
      Due to limitations in the aggregates class the current version of structured aggregation only performs piece-wise constant aggregation. Adding aggregation for piece-wise linear interpolation should be easy enough once the aggregates class is updated.
    \item \todo{Luc}{new interpolation based transfer operator factory, due Aug 14th}\\
      After updating both aggregates and structured aggregation classes \muelu will be ready for a new prolongator factory that will essentially perform the same tasks as GeneralGeometricPFactory but in a more modular way. This would complete the work on prolongators and will allows us to test piece-wise constant and piece-wise linear interpolation algorithm in the region framework.
    \end{enumerate}
\end{enumerate}

